Context-Aware Local Differential Privacy

Local differential privacy (LDP) is a strong notion of privacy for individual users that often comes at the expense of a significant drop in utility. The classical definition of LDP assumes that all elements in the data domain are equally sensitive. However, in many applications, some symbols are more sensitive than others. This work proposes a context-aware framework of local differential privacy that allows a privacy designer to incorporate the application's context into the privacy definition. For binary data domains, we provide a universally optimal privatization scheme and highlight its connections to Warner's randomized response (RR) and Mangat's improved response. Motivated by geolocation and web search applications, for $k$-ary data domains, we consider two special cases of context-aware LDP: block-structured LDP and high-low LDP. We study discrete distribution estimation and provide communication-efficient, sample-optimal schemes and information-theoretic lower bounds for both models. We show that using contextual information can require fewer samples than classical LDP to achieve the same accuracy.

==> fig_new.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[thick, scale = 3.5]
\begin{scope}[fill opacity=0.5]
\fill[fill=red!50] 
    plot[smooth,samples=100,domain=0:0.25] (\x,{1 - \x}) -- 
    plot[smooth,samples=100,domain=0.25:0] (\x,{1-3*\x});

\fill[fill=red!50] 
    plot[smooth,samples=100,domain=0.25:1] (\x,{1 - \x}) -- 
    plot[smooth,samples=100,domain=1:0.25] (\x,{(1-\x)/3});

\draw[domain=0:0.25] plot (\x,{1 - 3*\x});

\draw[domain=0.25:1] plot (\x,{(1 - \x)/3});


\fill[fill=blue!50] 
    plot[smooth,samples=100,domain=0:1/7] (\x,{1 -\x}) -- 
    plot[smooth,samples=100,domain=1/7:0] (\x,{1-4*\x});

\fill[fill=blue!50] 
    plot[smooth,samples=100,domain=1/7:1] (\x,{1 - \x}) -- 
    plot[smooth,samples=100,domain=1:1/7] (\x,{(1-\x)/2});


\draw[domain=0:1/7] plot (\x,{1 - 4*\x});

\draw[domain=1/7:1] plot (\x,{(1 - \x)/2});

\end{scope}

\draw [dashed] (0,0)--(0.6,0.6);
\draw (1pt,0.25)--(-1pt,0.25) node[left] {$\frac{1}{1+e^\eps}$}; 
\draw (0.25,1pt)--(0.25,-1pt) ;
\node at (0.3, -0.08) {$\frac{1}{1+e^\eps}$};
\draw [dashed] (0.25,0) -- (0.25, 0.25);
\draw [dashed] (0,0.25) -- (0.25, 0.25);
%labels 
\node at (-0.05, -0.05) {$0$};
%\node at (0.5, -0.4) {(a) Error Region for Standard LDP.};

%coordinate grid
\draw (0,0)--(1.05,0) node[right]{$P_{\rm MD}$};
\draw (0,0)--(0,1.05) node[above]{$P_{\rm FA}$};
\foreach \x in {1}
    \draw (\x,1pt)--(\x,-1pt) node[below] {$\x$};
\foreach \y/\ytext in {1}
    \draw (1pt,\y)--(-1pt,\y) node[left] {$\y$};  

\draw (1pt,3/7)--(-1pt,3/7) node[left] {$\frac{e^{\eps_{x',x}} -1}{e^{\eps_{x,x'}+\eps_{x',x}}-1}$}; 
\draw (1/7,1pt)--(1/7,-1pt);
\node at (1/7, -0.21) {$\frac{e^{\eps_{x,x'}} -1}{e^{\eps_{x,x'}+\eps_{x',x}}-1}$};
\draw [dashed] (1/7,0) -- (1/7, 3/7);
\draw [dashed] (0,3/7) -- (1/7, 3/7);
%labels 
%\node at (0.5, -0.4) {(b) Error Region for Context-Aware LDP.};
\end{tikzpicture}
\vspace{-10pt}
\caption{Error region for hypothesis testing between $x$ and $x'$ under DP constraints when $\eps_{x, x^\prime} < \eps_{x^\prime,x}$. (Blue for Context Aware LDP, Red for standard LDP)}
\vspace{-9pt}
\label{fig:err_region}
\end{figure}


==> k-ary_old.tex <==
\section{$k$-ary Alphabet} \label{sec:k_ary}

For general generalizations to the $k$-ary alphabet, unlike the binary case, it is not clear whether there exists an optimal scheme for all. One easy observation is that, for any matrix $\Epsilon$, let $\eps^* = \min_{i,j} \eps_{i,j}$, then any $\eps^*$-LDP algorithm will also satisfy $\Epsilon$-LDP. But this is not interesting since this won't help us get rid of the stringent requirement of standard LDP. Hence it would be more reasonable for us to consider some special $\Epsilon$ matrices which are both practically interesting and easier to implement.

What are the interesting $\Epsilon$'s to consider? First it is easy to observe that $\forall i \neq j \neq l \in [k]$, it is reasonable to assume that 
\begin{equation}\label{eqn:triangle}
	\eps_{i,j} \le \eps_{i,k} + \eps_{k,j}
\end{equation}

since any algorithm should satisfy:
\[
	\frac{\probof{Y = y|X = i}}{\probof{Y = y|X = j}} = \frac{\probof{Y = y|X = i}}{\probof{Y = y|X = k}} \frac{\probof{Y = y|X = k}}{\probof{Y = y|X = j}} \le e^{\eps_{i,k} + \eps_{k,j}}.
\]

Another principle for designing $\Epsilon$ matrices is that we want to have as few parameters as possible since we want our model to be easy to use and have good operational meanings. Under these two principles, we consider the following generalization of Block-Structured LDP
which has good operational meaning in real world applications such as geolocation data. And in Section~\ref{sec:dist_est}, for the task of distribution estimation, we will design algorithms that are easy to implement and study how these privacy constraints would affect the information-theoretic performance.
\todos{Good operational meanings for this case.}

\subsection{Block-Structured LDP}

In this section, we describe a new generalized definition of Local Differential Privacy(LDP), Block-Structured LDP (BSLDP).

\begin{definition}
	Let $f: \cX \rightarrow \cY$ be a randomized function. Suppose there is a partition of $\cX$, which is $\cP = \{ \cX_1, \cX_2, ..., \cX_m \}$. Then $\forall  \eps$, $f$ is $(\cP, \eps)$ - BSLDP if it satisfies $\forall i \in [m]$, $x_1, x_2 \in \cX_i$, and any $S \subset \cY$, we have:
	\[
	\frac{\probof{f(x_1) \in S}}{\probof{f(x_2) \in S}} \le e^{\eps}
	\]
	
\end{definition}

This definition relaxes the local version of differential privacy in the following way: Given a partition of the input set $\cP = \{ \cX_1, \cX_2, ..., \cX_m \}$, it requires different levels of indistinguishablitity for element pairs in the same block and those in different blocks. When $\eps_2 = \eps_1$, we recover the classic definition of LDP. Generally $\eps_2 \gg \eps_1$, which means we require stronger privacy guarantee within blocks compared to inter block pairs. The can be motivated from map applications, where it is acceptable to reveal the current city that someone is in while revealing the exact street address can be prohibitive. If $\eps_2 = \infty$, we don't have any privacy guaruntees on revealing which block the sample lies in.

\subsection{Distribution Learning under BS-LDP}  \label{sec:dist_est}
In this section, we consider the problem of distribution estimation under block-structured LDP constraints. In particular, we will prove the following theorem:


\begin{theorem} \label{thm:bs_complexity}
	Let $\cP = \{ \cX_1, \cX_2, ..., \cX_m \}$ be a partition of $\cX$ and $\cW_{\cP, \eps}$ be set of all possible channels that satisfy $(\cP, \eps)$-BSLDP, then:
	\[
	n(k,\alpha,\cW_{\cP,\eps}) = \Theta \Paren{\frac{\sum_{i=1}^m k_i^2}{\alpha^2 \eps^2}},
	\]
	where $\forall i \in [m], |\cX_i| = k_i$ and $|\cX| = k = \sum_{i=1}^{m} k_i$.
\end{theorem}

We can see that when we have $m$ blocks of equal size being $\frac{k}{m}$, we get the sample complexity will be $\Theta \Paren{\frac{k^2}{m\alpha^2 \eps^2}}$, which is a factor of $m$ less than the sample required for standard LDP. We give an algorithm based on HR that is $(\cP, \eps)$ - BS LDP, and using $n$ samples and $\log k$ bits of communication from each user, the algorithm can learn the distribution up to TV distance:
\begin{equation} \label{eqn:bs_l1}
O \Paren{ \sqrt{\frac{\sum_{i = 1}^m k^2_i}{n \eps^2} }}
\end{equation}

We also prove a matching lower bound which shows that our algorithm is also information theoretically optimal. Due to space limitations, we only briefly describe the encoding scheme.

\subsubsection{Block Hadamard Response.} \label{sec:bs_upper}
The idea of the algorithm is the perform Hadamard Response provided in~\cite{AcharyaSZ19} inside each block. For each block $B_j, j\in [m]$, we associate a hadamard matrix $H_{K_j}$ with $K_j = 2^{\ceil{\log {k_j+1}}} $. Let $\cY_j = \{(j, i) | i \in [K_j]\}$. For each $i \in B_j$, we assign a row of $H_{K_j}$ to $i$. Define the set of locations of $'+1'$'s to be $S_i$.  Then the whole output set will be $\cup_{j =1}^m \cY_j$. Then encoding scheme is defined as:
\[
Q(Y = (j,i)| X) = 
\begin{cases}
\frac{2e^\eps }{K_j (1 + e^\eps)},& X \in B_j, i \in S_X \\
\frac{2}{K_j (1 + e^\eps)},& X \in B_j, i \notin S_X \\
0, & \text{elsewhere.} 
\end{cases} 
\]

The decoding will follow similar spirit as in~\cite{AcharyaSZ19}. We ignore details and proofs for the lack of space.

==> related_work.tex <==
Local differential privacy (LDP) is an adaptation of central DP to the local setting where all pairs of elements in a data domain are equally sensitive. Such a formulation has the advantage of providing context-free, worst-case privacy guarantees but often leads to a significant reduction in utility. This work introduces a general context-aware notion of local privacy where different pairs of elements can have different sensitivity levels. For binary domains, we provide a universal optimality result and highlight precise (and interesting) connections to Warner's response and Mangat's improved response. For $k$-ary domains, we look at a canonical context-aware generalization where the domain is partitioned into sets and the goal is to make it hard to distinguish elements within the same set. For example, in geolocation applications, users can be in different cities, and it is not important to hide the city of a person as much as where exactly in that city a person is (i.e., which bars, restaurants, or businesses that person visits). In other words, in this context, users would like to hide which element in a given partition of the domain their data belongs to -- and not necessarily which partition the data is in because it may be obvious from the context of the application or side information. 

We consider the canonical task of distribution estimation, and under both models, we provide tight utility-privacy trade-offs. We also show that a modified version of the recently introduced optimal Hadamard Response is utility and communication optimal under these settings. 
\paragraph{Related work}
Local Differential Privacy can be dated back to~~\cite{warner1965randomized} and has gathered interest recently since~\cite{Dwork06, BeimelNO08, KasiviswanathanLNRS11}. The definition requires each user to send a randomized version of the data to the server and provides rigorous privacy guarantee even without a trusted curator. However, this often comes with the cost of a drop in the utility. 

Distribution estimation, where given independent samples from an unknown distribution, the goal is to estimate the underlying distribution up to a certain accuracy, has been studied since long ago~\cite{BarlowBBB72, DG85, Silverman:86, DevroyeL01}. The study of the tradeoff between utility and privacy for the problem of distribution estimation has gathered much attention recently and optimal rates have been established~\cite{duchi2013local, DiakonikolasHS15, kairouz2016discrete, WangHWNXYLQ16, YeB17, AcharyaSZ19}. They have showed that the sample complexity for $k$-ary distribution estimation up to accuracy $\alpha$ has increased from $\Theta \Paren{\frac{k}{\alpha^2}}$ to $\Theta\Paren{\frac{k^2}{\alpha^2 \eps^2}}$ if we impose $\eps$-LDP constraints.

Another line of work considers a similar but slightly different problem of heavy hitter estimation where there is no distributional assumption under the samples and the main focus is on reducing the computational complexity~\cite{bassily2015local, BassilyNST17, hsu2012distributed, wang2017locally, BunNS18, zhu2019federated, AcharyaS19}.

LDP imposes the same, context-agnostic privacy guarantee on each element in the alphabet. There are some works trying to relax the definition of DP~\cite{chatzikokolakis2013broadening, doudalis2017one, borgs2018revealing} and LDP~\cite{chatzikokolakis2017efficient, Alvim2018InvitedPL,murakami2018restricted} based on the structure of the underlying alphabet. \cite{doudalis2017one, murakami2018restricted} defines a secret set and only requires the probability of guessing an element in an secret set cannot increase too much. \cite{chatzikokolakis2013broadening, borgs2018revealing, chatzikokolakis2017efficient, Alvim2018InvitedPL} induces a metric over the underlying space and define the privacy parameter between each pair based on their distance over the metric space. 
